Template-Based Financial Report Generation in Agentic and Decomposed Information Retrieval

Tailoring structured financial reports from companies' earnings releases is crucial for understanding financial performance and has been widely adopted in real-world analytics. However, existing summarization methods often generate broad, high-level summaries, which may lack the precision and detail required for financial reports that typically focus on specific, structured sections. While Large Language Models (LLMs) hold promise, generating reports adhering to predefined multi-section templates remains challenging. This paper investigates two LLM-based approaches popular in industry for generating templated financial reports: an agentic information retrieval (IR) framework and a decomposed IR approach, namely AgenticIR and DecomposedIR. The AgenticIR utilizes collaborative agents prompted with the full template. In contrast, the DecomposedIR approach applies a prompt chaining workflow to break down the template and reframe each section as a query answered by the LLM using the earnings release. To quantitatively assess the generated reports, we evaluated both methods in two scenarios: one using a financial dataset without direct human references, and another with a weather-domain dataset featuring expert-written reports. Experimental results show that while AgenticIR may excel in orchestrating tasks and generating concise reports through agent collaboration, DecomposedIR statistically significantly outperforms AgenticIR approach in providing broader and more detailed coverage in both scenarios, offering reflection on the utilization of the agentic framework in real-world applications.

==> sections/6-limitations.tex <==
\section{Limitations}
The limitations of our work include the following aspects:
\begin{enumerate}
\item Query decomposition in DecomposedIR requires manual design, which limits its ability to generalize well. In future work, we aim to replace manual decomposition with LLM-based query decomposition, allowing for more flexible and scalable generalization.

\item Since our work lacks a ground truth for evaluation, current evaluation methods mostly rely on reference-free approaches. In our future work, we plan to involve domain experts to assess the quality of and differences between AgenticIR and DecomposedIR.

\item Due to the absence of pre-labeled ground truth for validating the relevance of the retrieved chunks, we assume the retrieved chunks are correct for the purposes of this study. We leave the exploration for validating or improving the accuracy of the retrieval process as future work.
\end{enumerate}

==> tables/tab1-4omini_original.tex <==
\begin{table}
\small
% \centering
\caption[c]{DecompEval (GPT-4o-mini) of AgenticIR \& DecomposedIR (A stands for AgenticIR; D stands for DecomposedIR).}
\setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{0.9}
\begin{tabular}{l|p{1.5cm} p{1.5cm} p{1.5cm} p{1.6cm}}
\toprule
% \cmidrule{3-5}
% \multirow{2}{*}{Category} & \multicolumn{2}{c|}{Details} & \multirow{2}{*}{Total} \\
Comp. & Financial Takeaways & Financial Context & Reasoning Correctness & Management Expectation \\
\midrule
INTC (A) & 0.27 & 0.44 & 0.79 & 0.24 \\
INTC (D) & 0.28 & 0.52 & 0.92 & 0.25 \\
\midrule
GFS (A) & 0.42 & 0.57 & 0.79 & 0.27 \\
GFS (D) & 0.37 & 0.62 & 0.90 & 0.30 \\
\midrule
SSNLF (A) & 0.18 & 0.26 & 0.59 & 0.14 \\
SSNLF (D) & 0.19 & 0.44 & 0.91 & 0.23 \\
\midrule
TSM (A) & 0.28 & 0.32 & 0.68 & 0.28 \\
TSM (D) & 0.29 & 0.43 & 0.91 & 0.25 \\
\midrule
UMC (A) & 0.34 & 0.42 & 0.72 & 0.20 \\
UMC (D) & 0.32 & 0.52 & 0.92 & 0.31 \\
\specialrule{0.15em}{0.1em}{0.25em}
Avg. (A) & \textbf{0.30} & 0.40 & 0.71 & 0.22 \\
Avg. (D) & 0.29 & \textbf{0.50} & \textbf{0.91} & \textbf{0.26} \\
\bottomrule
\end{tabular}
\label{tab:DecompEval_gpt}
\end{table}

==> tables/tab2-llama405b.tex <==
\begin{table}
\small
% \centering
\caption[c]{DecompEval (Llama-3.1-405B) of AgenticIR \& DecomposedIR. Due to the length of TSM's earnings call exceeding the input limit of SambaNova's Llama-3.1 model, results are reported only for the other four companies.}
% Due to the length of TSM's earnings call exceeding the input limit of SambaNova's Llama-3.1 model, results are reported only for the other four companies. (A: AgenticIR, D: DecomposedIR) A stands for AgenticIR, D stands for DecomposedIR
\setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{0.9}
\begin{tabular}{l|p{1.5cm} p{1.5cm} p{1.5cm} p{1.6cm}}
\toprule
% \cmidrule{2-5}
Comp. & Financial Takeaways & Financial Context & Reasoning Correctness & Management Expectation \\
\midrule
INTC (A) & 0.29 & 0.21 & 0.56 & 0.25 \\
INTC (D) & 0.27 & 0.34 & 0.80 & 0.23 \\
\midrule
GFS (A) & 0.43 & 0.38 & 0.68 & 0.25 \\
GFS (D) & 0.35 & 0.40 & 0.78 & 0.24 \\
\midrule
SSNLF (A) & 0.17 & 0.19 & 0.55 & 0.13 \\
SSNLF (D) & 0.16 & 0.34 & 0.86 & 0.19 \\
\midrule
UMC (A) & 0.38 & 0.27 & 0.65 & 0.18 \\
UMC (D) & 0.30 & 0.38 & 0.83 & 0.24 \\
\specialrule{0.15em}{0.1em}{0.25em}
Avg. (A) & \textbf{0.31} & 0.26 & 0.61 & 0.19 \\
Avg. (D) & 0.27 & \textbf{0.36} & \textbf{0.81} & \textbf{0.22} \\
\bottomrule
\end{tabular}
% \begin{tablenotes}
% \footnotesize
% \item Note: Due to the length of TSM's earnings call exceeding the input limit of SambaNova's Llama-3.1 model, we only computed results for the other four companies.
% \end{tablenotes}
\label{tab:DecompEval_llama}
\end{table}

==> tables/tab3-characteristic.tex <==
\begin{table}
% \small
\footnotesize
% \vspace{-5pt}
\caption[c]{Four Specific Characteristics}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{0.9}
\resizebox{0.95\linewidth}{!}{
% \begin{tabular}{p{1.87cm}|p{6.4 cm}}
\vspace{-5pt}
\begin{tabular}{lc}
\toprule
\textbf{Characteristic} & \textbf{Description} \\
\midrule
% \cmidrule{2}
\makecell[l]{Financial\\Takeaways} & \makecell[l]{Key financial details or numerical statistics related to\\the company's performance this quarter} \\
\hline
\makecell[l]{Financial\\Context} & \makecell[l]{Company's current financial performance, such as\\references to previous quarters} \\
\hline
\makecell[l]{Reasoning\\Correctness} & \makecell[l]{Accurate reasoning or explanations for the company's\\financial performance this quarter} \\
\hline
\makecell[l]{Management\\Expectation} & \makecell[l]{Expectations or projections about the company's future\\performance or next quarter} \\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
\label{tab:characteristic}
\end{table}

==> tables/tab5-Agent_prompt.tex <==
% \begin{table*}
% \small
% \caption[c]{System Prompts in AgenticIR}
% \begin{tabular}{l|l}
% \toprule
% Agent & System Prompts \\
% \midrule
% Generate & \makecell[l]{You are a helpful AI Assistant.
% You can interact with Assistant to complete the task.
% Reply 'TERMINATE' if\\ all sub-tasks are completed.}\\
% \midrule
% Assistant Agent &  \makecell[l]{You are a helpful AI assistant.
% You can use the task planner to decompose a complex task into sub-tasks.
% You\\ can also use the retrieve data to get earnings call transcript by subqueries you generate based on sub-tasks.\\
% Make sure to follow through with the subqueries.
% Follow the template to generate the financial report in text\\ format. 
% Add or Return 'TERMINATE' only if the final report is completed.}\\
% \bottomrule
% \end{tabular}
% \label{tab:agent_prompt}
% \end{table*}

\begin{table*}
% \small
\centering
\caption[c]{System Prompts of AgenticIR.}
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{0.9}
% \begin{tabular}{l|p{0.85\textwidth}}
\begin{tabular}{l|l}
% \begin{longtable}{l|p{12cm}}
\toprule
% \cmidrule{2-5}
Agent & System Prompts \\
\midrule
User Proxy Agent & \makecell[l]{You are a helpful AI Assistant.
You can interact with Assistant to complete the task.
Reply\\ 'TERMINATE' if all sub-tasks are completed.}\\
\midrule
Assistant Agent &  \makecell[l]{You are a helpful AI assistant.
You can use the task planner to decompose a complex task into\\ sub-tasks.
You can also use the retrieve data to get earnings call transcript by subqueries you\\ generate based on sub-tasks.
Make sure to follow through with the subqueries.
Follow the template\\ to generate the financial report in text format. 
Add or Return 'TERMINATE' only if the final report\\ is completed.}\\
\midrule
Financial Retrieval Agent & You are financial retriever, a content retrieval assistant.
Retrieve financial data from external resources.\\
\midrule
Financial Manager & You are the financial manager. Your responsibility is to answer the question given the retrieved context.\\
\midrule
Task Decompose Agent & \makecell[l]{You are a helpful AI assistant. 
You suggest a feasible plan for finishing a complex task by\\ decomposing it into lots of sub-tasks.}\\
\bottomrule
\end{tabular}
% \end{longtable}
\label{tab:agent_prompt}
\end{table*}

==> tables/tab6_decompIR_prompt.tex <==
\begin{table*}
% \small
\centering
\caption[c]{LLM Prompts in DecomposedIR.}
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{0.9}
% \begin{tabular}{l|p{0.85\textwidth}}
\begin{tabular}{l|l}
% \begin{longtable}{l|p{12cm}}
\toprule
% \cmidrule{2-5}
Action & LLM Prompts \\
\midrule
Generate & \makecell[l]{You are a senior financial analyst. Based on the provided context (earnings call transcript) and financial\\
statement JSON, try  to answer the question and the numerical value as precise as possible based on\\ the provided context. Ensure clarity and CONCISENESS in the response.\\
Transcript Relevant Context:\\
\textit{\{context\}}\\
Financial Statement JSON:\\
\textit{\{statement\}}\\
Question:\\
\textit{\{question\}}}\\
\midrule
Summarize &  \makecell[l]{I will provide several questions along with their corresponding answers and the reasoning behind those answers,\\
as well as the section to summarize. Please summarize the answers into a single cohesive response focused on\\
this aspect, and consolidate the reasoning into a concise explanation. Ensure that all numerical data is accurately\\ 
preserved and aligned with the section. Do not include any external or speculative information.
The final\\
summarized response and explanation must be logically consistent, focused on the section, and aligned with\\
the provided content.\\
Questions and Answers:\\
\textit{\{question and answer\}}\\
Section to Summarize\\
\textit{\{section\}}\\
}\\
\bottomrule
\end{tabular}
% \end{longtable}
\label{tab:decomposed_prompt}
\end{table*}

==> tables/tab7-SumIPCC_DecompEval.tex <==
\begin{table}
\small
\caption[c]{DecompEval scores of AgenticIR, AgenticIR with self-reflection and DecomposedIR on the SumIPCC dataset across four characteristics.}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|>{\raggedright\arraybackslash}p{1.5cm} >{\raggedright\arraybackslash}p{1.5cm} >{\raggedright\arraybackslash}p{1.5cm} >{\raggedright\arraybackslash}p{1.5cm}}
\toprule
\textbf{Methods} & \textbf{Climate statistics} & \textbf{Human influence} & \textbf{Impacts on ecosystems} & \textbf{Future projections} \\
\midrule
AgenticIR & 0.09 & 0.12 & 0.35 & 0.16 \\
AgenticIR$_{sr}$ & 0.16 & 0.22 & 0.33 & 0.27 \\
DecomposedIR & 0.04 & 0.14 & 0.10 & 0.02 \\
\bottomrule
\end{tabular}
\label{tab:SumIPCC_DecompEval}
\end{table}


